Prioritizing Informative Features and Examples for Deep Learning from Noisy Data

In this dissertation, we propose a systemic framework that prioritizes informative features and examples to enhance each stage of the development process. Specifically, we prioritize informative features and examples and improve the performance of feature learning, data labeling, and data selection. We first propose an approach to extract only informative features that are inherent to solving a target task by using auxiliary out-of-distribution data. We deactivate the noise features in the target distribution by using that in the out-of-distribution data. Next, we introduce an approach that prioritizes informative examples from unlabeled noisy data in order to reduce the labeling cost of active learning. In order to solve the purity-information dilemma, where an attempt to select informative examples induces the selection of many noisy examples, we propose a meta-model that finds the best balance between purity and informativeness. Lastly, we suggest an approach that prioritizes informative examples from labeled noisy data to preserve the performance of data selection. For labeled image noise data, we propose a data selection method that considers the confidence of neighboring samples to maintain the performance of the state-of-the-art Re-labeling models. For labeled text noise data, we present an instruction selection method that takes diversity into account for ranking the quality of instructions with prompting, thereby enhancing the performance of aligned large language models. Overall, our unified framework induces the deep learning development process robust to noisy data, thereby effectively mitigating noisy features and examples in real-world applications.

==> part1_TAUFE/2_related_work.tex <==
\section{Background and Related Work}
\label{sec:related_work}

\textbf{Negative Impact of Undesirable Features.}
\hspace{0.1cm} DNNs tend to overly capture all available signals from training data even when they are not essential for solving a given task\,\cite{wang2020high, ilyas2019adversarial}. 
The occurrence of undesirable features and their negative impact have been recently witnessed in various types of learning tasks.
In image classification, a classification model often uses background or texture features as an undesirable shortcut for making a prediction instead of using the intrinsic shape of a target class\,\cite{ilyas2019adversarial,geirhos2018imagenet}.
In object detection, a detector model easily overfits to the background features for localizing target objects in a scene\,\cite{oksuz2020imbalance, singh2018analysis}.
In video action recognition, a recognition model often relies on static cues in a single frame rather than temporal actions over consecutive frames\,\cite{weinzaepfel2021mimetics, li2019repair}.
In natural language processing\,(NLP) tasks, a language model often makes its predictions based on frequent but meaningless words instead of using semantically meaningful words\,\cite{gururangan2018annotation}.

\textbf{Connection with Adversarial Examples.}\hspace{0.1cm} DNNs are easily deceived by adversarial perturbations of the inputs, so-called adversarial examples\,\cite{yuan2019adversarial}. Differently from standard learning, the undesirable features are maliciously added and then make the model incur more errors. In addition, it is widely known that such adversarial perturbations are transferable even from different domains\,\cite{naseer2019cross}; that is, an adversarial attack can drastically degrade the generalization capability of the classifier without knowing its internals\,\cite{naseer2019cross}. To remedy this problem, the use of OOD examples has gained great attention in that they enhance the robustness against the adversarial examples by preventing the model from overfitting to the undesirable features\,\cite{lee2021removing}. 

\textbf{Removing Undesirable Feature Contribution.}\hspace{0.1cm} 
Numerous studies have attempted to prevent overfitting to the undesirable features in standard supervised learning tasks.
A typical way is \emph{de-biasing}, which removes the undesirable feature contribution based on the pre-defined bias for the target task.
Geirhos et al.\,\cite{geirhos2018imagenet} took advantage of data augmentation techniques to generate de-biased examples from training data. 
Lee et al.\,\cite{lee2019srm} and Shetty et al.\,\cite{shetty2019not} synthesized de-biased examples by leveraging a generative model for image stylization or object removal. 
Wang et al.\,\cite{wang2018learning} quantified the local feature bias by using the neural gray-level co-occurrence matrix. 
Bahng et al.\,\cite{bahng2020learning} proposed a framework that leverages a bias-characterizing model to remove pixel-level local undesirable features. 
This family of methods successfully removes the \emph{pre-defined} bias from the undesirable features but is not generalizable to other types of bias. Even worse, it is hard to identify the types of undesirable features in advance since they are not comprehensible even to a human.

In this regard, motivated by the transferability of undesirable features in different domains, the usefulness of OOD examples for de-biasing started to be discussed. Although the representative softmax calibrator, OAT\,\cite{lee2021removing}, does not need a pre-defined bias type, it suffers from two limitations, lack of flexibility and feature entanglement. Many aspects, such as high generalizability and in-depth theoretical analysis, are yet to be explored.


==> part2_MQNet/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Active Learning and Open-set Recognition}
\label{sec:active_learning}

\textbf{Active Learning} is a learning framework to reduce the human labeling cost by finding the most {informative} examples given unlabeled data\,\cite{ren2021survey, park2022active}.
One popular direction is uncertainty-based sampling.
Typical approaches have exploited prediction probability, \textit{e.g.}, soft-max confidence\,\cite{lewis1994heterogeneous, wang2014active}, margin\,\cite{roth2006margin}, and entropy\,\cite{joshi2009multi}.
Some approaches obtain uncertainty by Monte Carlo Dropout on multiple forward passes\,\cite{gal2017deep, kirsch2019batchbald, gal2016dropout}.
LL\,\cite{yoo2019learning} predicts the loss of examples by jointly learning a loss prediction module with a target model.
Meanwhile, diversity-based sampling has also been widely studied.
To incorporate diversity, most methods use a clustering\,\cite{nguyen2004active, citovsky2021batch} or coreset selection algorithm\,\cite{sener2018active}.
Notably, CoreSet\,\cite{sener2018active} finds the set of examples having the highest distance coverage on the entire unlabeled data.
BADGE\,\cite{Ash2020badge} is a hybrid of uncertainty- and diversity-based sampling which uses $k$-means{++} clustering in the gradient embedding space.
However, this family of approaches is not appropriate for open-set AL since they do not consider how to handle the OOD examples for query selection.\looseness=-1

\textbf{Open-set Recognition (OSR)} is a detection task to recognize the examples outside of the target domain\,\cite{geng2020recent}. Closely related to this purpose, OOD detection has been actively studied\,\cite{yang2021generalized}. 
Recent work can be categorized into classifier-dependent, density-based, and self-supervised approaches.
The classifier-dependent approach leverages a pre-trained classifier and introduces several scoring functions, such as Uncertainty\,\cite{MSP}, ODIN\,\cite{ODIN}, Mahalanobis distance\,(MD)\,\cite{MD}, and Energy\cite{ENERGY}.
Recently, ReAct\,\cite{sun2021react} shows that rectifying penultimate activations can enhance most of the aforementioned classifier-dependent OOD scores.
The density-based approach learns an auxiliary generative model like a variational auto-encoder to compute likelihood-based OOD scores\,\cite{, ren2019likelihood, serra2019input, DGM}.
Most self-supervised approaches leverage contrastive learning\,\cite{tack2020csi, winkens2020contrastive, sehwag2021ssd}.
CSI shows that contrasting with distributionally-shifted augmentations can considerably enhance the OSR performance\,\cite{tack2020csi}.

The OSR performance of classifier-dependent approaches degrades significantly if the classifier performs poorly\,\cite{vaze2021open}. Similarly, the performance of density-based and self-supervised approaches heavily resorts to the amount of clean IN data\,\cite{DGM, tack2020csi}.
Therefore, open-set active learning is a challenging problem to be resolved by simply applying the OSR approaches since it is difficult to obtain high-quality classifiers and sufficient IN data at early AL rounds.

\subsection{Open-set Active learning}
\label{sec:open-active_learning}

Two recent approaches have attempted to handle the open-set noise for AL\,\cite{du2022conal, kothawade2021similar}.
Both approaches try to increase purity in query selection by effectively filtering out the OOD examples.
CCAL\,\cite{du2022conal} learns two contrastive coding models each for calculating informativeness and OODness of an example, and  combines the two scores using a heuristic balancing rule.
SIMILAR\,\cite{kothawade2021similar} selects a pure and core set of examples that maximize the distance on the entire unlabeled data while minimizing the distance to the identified OOD data.
%
However, we found that CCAL and SIMILAR are often worse than standard AL methods since they always put higher weights on purity although informativeness should be emphasized when the open-set noise ratio is small or in later AL rounds.
This calls for developing a new solution to carefully find the best balance between purity and informativeness.




==> part3_Prune4ReL/2-relatedwork.tex <==
\section{Preliminary and Related Work}
\label{sec:related_work}


\subsection{Robust Learning under Noisy Labels}
\label{sec:robust_learning_under_noisy_labels}

A long line of literature has been proposed to improve the robustness of DNNs against label noise -- refer to \cite{song2022learning} for a detailed survey for deep learning with noisy labels.
While some studies have focused on modifying the architectures\,\cite{goldberger2017training, han2018masking, yao2018deep} and the loss functions\,\cite{ghosh2017robust, hendrycks2018using, ma2020normalized}, others have opted for sample selection approaches\,\cite{jiang2018mentornet, han2018co, wei2020combating, wu2020topological} that select as many clean examples as possible while discarding noisy examples based on some cleanness criterion, such as small-loss\,\cite{han2018co}. %, in order to train a noise-vulnerable standard classifier on the clean sample set.
Note that, these works do not consider the compactness or efficiency of the selected sample set. 
%mainly focus on improving model generalization performance and 
Meanwhile, to further exploit even noisy examples for training, \emph{Re-labeling}\,\cite{song2019selfie, zhou2021robust} approaches try to correct noisy labels and use them for training with a re-labeling module, e.g., a heuristic rule\,\cite{song2019selfie}.% or a regularizer.
% of the suspected noisy examples 
Notably, according to recent benchmark studies on real-world noisy datasets\,\cite{wei2021learning}, a family of Re-labeling methods with \emph{self-consistency regularization}\,\cite{xie2020unsupervised} has shown state-of-the-art performance.


%\textbf{Re-labeling} \ 
In general, Re-labeling with self-consistency regularizer is based on the following optimization form:
\begin{equation}
\begin{gathered}
\mathcal{L}_{{Re\text{-}labeling}}(\tilde{\mathcal{D}}; \theta,\!\mathcal{A})=\sum_{(x,\tilde{y}) \in \tilde{\mathcal{D}}} \mathbbm{1}_{[{C}_{{\theta}}(x)\ge\tau]} \mathcal{L}_{ce}(x,\tilde{y};{\theta})+\lambda ~\!\sum_{x \in \tilde{\mathcal{D}}}\mathcal{L}_{reg}(x;{\theta},\!\mathcal{A}),
\end{gathered}
\label{eq:relabeling}
\end{equation}
where $\mathcal{\tilde{D}}=\{(x_i, \tilde{y}_i)\}_{i=1}^{m}$ is a given noisy training set obtained from a noisy joint distribution $\mathcal{X} \times \mathcal{\tilde{Y}}$, ${\theta}$ is a classifier, $\mathcal{A}$ is a strong data augmentation, $\mathcal{C}_{{\theta}}(\cdot)$ is a prediction confidence score, and $\tau$ is a threshold to identify confident (clean) examples for the supervised loss $\mathcal{L}_{ce}(x,\tilde{y};{\theta})$, i.e., cross-entropy. The noisy labels are implicitly corrected by the self-consistency loss $\mathcal{L}_{reg}(x;{\theta})$ exploiting the power of strong augmentations\,\cite{cubuk2020randaugment}.
DivideMix\,\cite{li2020dividemix}, ELR+\,\cite{liu2020early}, CORES\,\cite{cheng2020learning}, SOP+\,\cite{liu2022robust} are popular approaches belonging to this family.
%DivideMix splits the noisy data into labeled and unlabeled sets and applies the semi-supervised technique MixMatch\,\cite{}. 
%SOP+\,\cite{}, similarly, incorporates the self-consistency loss with additional learnable variables.
DivideMix uses a co-training framework to further improve re-labeling accuracy and SOP+ introduces additional learnable variables combined with self-consistency loss.
For simplicity, we call this Re-labeling family with self-consistency regularization as ``Re-labeling'' throughout the paper.
Despite their effectiveness, Re-labeling tends to require more computation time due to additional data augmentations, multiple backbones, and longer training epochs, which raises the need to study a new data pruning approach for enhancing its efficiency.
%a data pruning approach to enhance its efficiency has not yet been studied.


\begin{comment}
%DY
% Background, Recent Trends (Million $\&$ Billion scale)
% Sample Selection

% 많은 Noisy label Work들이 개발되었다 [Survey]
% 아키텍쳐 [ [16], [75]–[82].], Robust loss function [[68], [97]–[101].], Clean Sample Selection [[19], [70], [99], [112], [131]–[137] ], Re-labeling [DivideMix, ELR+, SOP, CORES] 
% % % % 또, Clean Sample Selection []이 있는데, 가능한 clean core함에 대한 고려는 없기 때문에 data pruning 성능 측면에서 optimal 은 아님.
% In practice, Re-labeling [] 이 모든 데이터를 fully explore하기 때문에, 가장 성능이 높은걸로 report 되고있다.
% 자세한건 refer to the survey
% \textbf{Re-labeling} 
% Relabeling is SOTA with self-consistency regularization
% 공통점: self-consistency regularization을 사용해서 automatic re-labeling
% DivideMix, ELR+, SOP, 
% 언급: more data augmentation, multiple backbones, longer epochs 특징 때문에, standard learning 보다 오래걸림 → data pruning 중요함

There have been many approaches to improve the robustness of DNNs against label noise. While some studies have focused on modifying the architecture\,\cite{} and the loss functions\,\cite{}, others have opted for \textit{clean sample selection} approaches\,\cite{} that select small-loss examples whose labels are likely to be true-labeled and train a DNN on the selected samples. Furthermore, more recent studies have shown that \textit{Re-labeling} methods\,\cite{}, which use the whole data by correcting the labels of the unselected samples to reliable ones, achieve state-of-the-art performances. SELFIE\,\cite{} corrects the labels of refurbishable examples according to the consistency of predictions.


\textbf{Re-labeling} \quad These Re-labeling methods have become more impressive by reducing the risk of false corrections through the use of self-consistency regularization. Let $\mathcal{\tilde{D}}=\{(x_i, \tilde{y}_i)\}_{i=1}^{m}$ be a given noisy training set obtained from a noisy joint distribution $\mathcal{X} \times \mathcal{\tilde{Y}}$, where $\tilde{y}\in \mathbb{R}^k$ denotes a noisy label in $k$-way classification. % and $m$ denotes the number of training examples. , and $S$ be a pruned subset
Here, Re-labeling methods split $\mathcal{\tilde{D}}$ into a re-labeled set $\mathcal{R}$, and an unlabeled set $\mathcal{U}$. % a clean set $\mathcal{C}$, 
The loss function of standard Re-labeling methods can be written as:
\begin{equation}
\begin{gathered}
\ell_{Re-labeling}=\sum_{(x,\hat{y}) \in \mathcal{{R}}} \ell_{CE}(x,\hat{y};\theta)+\lambda ~\!\sum_{x \in \mathcal{{U}}}\ell_{reg}(x;\theta),
\end{gathered}
\label{eq:relabeling}
\end{equation}
where $\theta$ be a classification model trained by a Re-labeling method, $\hat{y}$ is a corrected label, $\lambda$ is a constant, and $\ell_{CE}$ and $\ell_{reg}$ are the cross-entropy and the self-consistency loss, respectively. 
% Also, let $\tilde{\theta}$ be a classification model trained by a Re-labeling method and $f_{\tilde{\theta}}(x)\!\in\!\mathbb{R}^k$ be its class prediction on an input example $x$. 

For example, DivideMix\,\cite{} splits the noisy data into labeled and unlabeled sets and applies the semi-supervised technique MixMatch\,\cite{} as the self-consistency regularization. 
% For example, DivideMix\,\cite{} splits the noisy data into labeled and unlabeled sets and applies the semi-supervised technique MixMatch\,\cite{}. 
SOP+\,\cite{}, similarly, incorporates popular consistency regularization technique from robust learning literature\,\cite{} while explicitly modeling the label noise with additional learnable variables.
% to separate the noise from each training example.
% SOP+: A holistic approach to semi-supervised learning; Learning to learn from noisy labeled data.
Despite their effectiveness, Re-labeling methods tend to require more computational resources due to additional data augmentations, multiple backbone models, and longer training epochs.
\end{comment}


\subsection{Data Pruning}
\label{sec:data_pruning}
% 공통점: hard한 샘플을 뽑겠다; generalization 관점에서 더 도움된다 라는 가정하에
% 많은 방식들이 개발되었다.
% Categorization & Summary
% limitation: only for clean dataset

% Goal
In order to achieve high generalization performance with a selected subset, general data pruning approaches often prioritize the selection of hard or uncertain examples. 
Specifically, \textit{uncertainty-based} methods\,\cite{wang2014active,roth2006margin,joshi2009multi}  favor the selection of lower-confidence examples over highly confident ones, as the former is assumed to be more informative than the latter.
Similarly, \textit{geometry-based} methods\,\cite{chen2012super, sener2018active} focus on removing redundant examples that are close to each other in the feature space, while \textit{loss-based} methods\,\cite{toneva2018empirical, paul2021deep, killamsetty2021grad, mirzasoleiman2020coresets} involve selecting the samples with high loss or gradient measured during training. Refer to \,\cite{guo2022deepcore} for a detailed survey of data pruning for deep learning.
However, in realistic scenarios where there are noisy examples present, these existing methods may not always be applicable, because such samples may also exhibit high uncertainty and could potentially be considered informative for training\,\cite{toneva2018empirical}.
A few works attempted to improve the robustness of sample selection against label noise\,\cite{killamsetty2021glister}, but it requires an additional clean validation set which is difficult to obtain in practice. 
Also, to the best of our knowledge, there has been no work to consider the effect of data pruning on state-of-the-art noise-robust learners such as Re-labeling.

%However, in realistic scenarios where there are noisy examples present, a recent work reported that the existing pruning methods are vulnerable to such noisy examples because such examples also exhibit high uncertainty thereby often being selected to the pruned set\,\cite{toneva2018empirical}.


\begin{comment}
\textit{Bi-level optimization-based} methods\,\cite{killamsetty2021glister}, on the other hand, consider the optimization of data pruning as the outer objective, and that of a DNN on the selected subset as the inner objective.
However, in realistic scenarios where there are noisy examples present, these existing methods may not always be applicable, because such samples may also exhibit high uncertainty and could potentially be considered informative for training.
\end{comment}

% % uncertainty
% Coleman et al.\,\cite{coleman2019selection} shows that the uncertainty-based scores, e.g., Confidence\,\cite{wang2014active}, Margin\,\cite{roth2006margin}, and Entropy\,\cite{joshi2009multi}, can be effective metrics for subset selection in that selecting lower confident examples is more helpful for model generalization than selecting higher confident ones.
% % geometric
% Some work used the geometric distance in the feature space to avoid selecting examples with redundant information. Herding\,\cite{chen2012super} incrementally extends the selected coreset by greedily adding a data example which can minimize the distance between the center of the coreset and that of the original training set. kCenterGreedy\,\cite{sener2018active} selects $k$ examples that maximize the distance coverage on the entire unlabeled data.
% % Loss/Error
% Recently, many approaches try to directly exploit the components of deep learning with given ground-truth labels.
% Forgetting\,\cite{toneva2018empirical} selects examples that are easy to be forgotten by the classifier, and it finds such samples by counting how frequently predicted label changes during several warm-up training epochs.
% GraNd\,\cite{paul2021deep} uses the average norm of gradient vector to measure the contribution of each examples for minimizing the training loss.
% GradMatch\,\cite{killamsetty2021grad} and CRAIG\,\cite{mirzasoleiman2020coresets} try to find an optimal coreset that its gradient can be matched with the gradient of full training set.
% % Bi-level
% Glister\,\cite{killamsetty2021glister} introduces a bi-level optimization framework that the outer loop is for selecting the coreset which can be solved by a greedy algorithm.
% Submodular functions, such as Graph Cut, Facility Location, and Log Determinant, which measure the diversity of information, have also been shown to be useful for data subset selection\,\cite{iyer2013submodular}.

==> part3_Prune4ReL/tables/confidence_metrics_noisy_ratio.tex <==
\begin{table*}[!t]
\noindent
\small
%\caption{Funny Table Examples.} 
\parbox{.4\textwidth}{%
\parbox{5.0cm}{
\vspace{0.4cm}
\caption{Effect of the confidence metrics on \algnamec{} with SOP+.}
\vspace{0.1cm}
\label{table:effect_of_meta_input}
}
\scriptsize
\begin{tabular}{c|c|c c c c}\toprule
\multirow{2}{*}{\makecell[c]{\!\!\!Dataset\!\!\!}}& \multirow{2}{*}{\makecell[c]{\!\!\!Conf. Metric\!\!\!}} & \multicolumn{4}{c}{Selection Ratio} \\
& & 0.2&0.4&0.6&0.8\\ \midrule
\multirow{2}{*}{\makecell[c]{\!\!\!CIFAR-10N\\(Worst)\!\!\!}}& MaxProb & 83.4&89.3&91.5&92.5\\
& DiffProb &83.1&89.2&91.6&92.5\\ \midrule
\multirow{2}{*}{\makecell[c]{\!\!\!CIFAR-100N\!\!\!}}& MaxProb & 49.0&59.1&64.1&65.7\\
& DiffProb &48.6&59.9&64.0&66.0\\ \bottomrule
\end{tabular}
%\begin{tabular}{c|c c c c}\toprule
%Dataset & \multicolumn{4}{c}{CIFAR-10N (Worst)} \\ 
%Select Ratio & 0.2 & 0.4 & 0.6 & 0.8\\ \midrule
%MaxConf & 0.2 & 0.4 & 0.6 & 0.8\\
%MaxMargin & 0.2 & 0.4 & 0.6 & 0.8\\ \midrule
%Dataset & \multicolumn{4}{c}{CIFAR-100N} \\ 
%MaxConf & 0.2 & 0.4 & 0.6 & 0.8\\
%MaxMargin & 0.2 & 0.4 & 0.6 & 0.8\\ \bottomrule
%\end{tabular}
}%
\parbox{.6\textwidth}{%
\parbox{8.0cm}{
\vspace{0.4cm}
\caption{Ratio of noisy examples in the selected subset.}
\vspace{0.1cm}
\label{table:effect_of_meta_input}
}
\scriptsize
\begin{tabular}{c|c c c c|c c c c}\toprule
Dataset & \multicolumn{4}{c|}{\underline{CIFAR-10N (Worst)}} & \multicolumn{4}{c}{\underline{CIFAR-100N}} \\
Sel. Ratio & 0.2 & 0.4 & 0.6 & 0.8 & 0.2 & 0.4 & 0.6 & 0.8 \\ \midrule
SmallL & 0.8 & 3.6 & 11.5 & 26.2 & 3.5 & 8.7 & 16.3 & 27.4 \\
Margin & 54.6 & 52.1 & 48.5 & 44.6 & 61.5 & 56.8 & 51.6 & 46.2 \\
kCenter & 40.0 & 41.1 & 41.6 & 42.1 & 37.5 & 38.7 & 39.9 & 40.4 \\
Forget & 37.7 & 38.8 & 39.2 & 40.2 & 37.9 & 34.6 & 33.0 & 36.8 \\
GraNd & 91.5 & 79.4 & 64.2 & 50.1 & 93.9 & 57.3 & 61.2 & 49.3 \\
\textbf{\algnamec{}} & 38.7 & 42.7 & 43.5 & 46.5 & 28.3 & 29.1 & 33.3 & 37.2 \\ \bottomrule
\end{tabular}
}%
\vspace*{-0.3cm}
\end{table*}




==> part3_Prune4ReL/tables/perf_tbl.tex <==
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.1}% make the row margin compact
\begin{table*}[t!]
% \small
% \tiny
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Performance comparison of sample selection baselines and \algnamec{} on CIFAR-10N and CIFAR-100N. The best results are in bold and the second bests are underlined.}
\vspace*{0.2cm}
% \resizebox{1.0\columnwidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}c|c|cccc|cccc|ccccc@{}}
\toprule
\multirow{3}{*}{\hspace{-0.0cm}\makecell[c]{ReLabel\\Models}\hspace{-0.10cm}}&\multirow{3}{*}{\makecell[c]{Pruning\\Methods}}& \multicolumn{8}{c|}{{\underline{CIFAR-10N}}} 
& \multicolumn{4}{c}{{\underline{CIFAR-100N}}}\\%\cline{3-14} 
% \addlinespace[0.6ex]
% \multicolumn{1}{c|}{\hspace{-0.20cm}\textbf{ReLabel}\hspace{-0.20cm}}
% \multicolumn{1}{c|}{\hspace{-0.10cm}\textbf{Pruning}\hspace{-0.20cm}} 
%\addlinespace[0.4ex]
& & \multicolumn{4}{c|}{{Random}} & \multicolumn{4}{c|}{{Worst}} & \multicolumn{4}{c}{{Noisy}} \\
%\addlinespace[-0.2ex]
%\multicolumn{1}{c|}{\hspace{-0.20cm}\textbf{Method}\hspace{-0.20cm}} 
%& \multicolumn{1}{c|}{\hspace{-0.10cm}\textbf{Method}\hspace{-0.20cm}} 
& & \multicolumn{1}{c}{\hspace{-0.20cm}{0.2}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.4}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.6}}
& \multicolumn{1}{c|}{\hspace{-0.20cm}{0.8}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.2}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.4}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.6}}
& \multicolumn{1}{c|}{\hspace{-0.20cm}{0.8}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.2}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.4}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.6}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.8}}
\\ \midrule
% # Standard ###############################################################
\multirow{3}{*}{\hspace{-0.0cm}{Standard}\hspace{-0.10cm}}                           
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Uniform\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.5}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.9}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{83.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.6}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.4}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{00}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
% \midrule
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}SmallL\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.1}\scalebox{0.75}{$\pm$4.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.0}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{70.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{80.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.1}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
%\midrule
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Forget\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.1}\scalebox{0.75}{$\pm$4.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.0}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{70.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{80.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.1}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
\midrule
% # DivideMix ###############################################################
\multirow{8}{*}{\hspace{-0.0cm}{DivMix}\hspace{-0.10cm}} 
\begin{comment}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Full\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
\\
\end{comment}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Uniform\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{87.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.9}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{83.2}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{88.5}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.4}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{30.5}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.3}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{57.5}\scalebox{0.75}{$\pm$1.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{58.6}\scalebox{0.75}{$\pm$0.9}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}SmallL\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.1}\scalebox{0.75}{$\pm$4.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.0}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{70.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{80.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.1}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{33.3}\scalebox{0.75}{$\pm$3.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{47.4}\scalebox{0.75}{$\pm$1.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{59.4}\scalebox{0.75}{$\pm$0.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{62.0}\scalebox{0.75}{$\pm$1.2}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Margin\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.5}\scalebox{0.75}{$\pm$2.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.5}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.3}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{75.1}\scalebox{0.75}{$\pm$0.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{85.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.2}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{17.1}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{30.8}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{46.3}\scalebox{0.75}{$\pm$2.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.2}\scalebox{0.75}{$\pm$1.3}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}kCenter\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.4}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{93.0}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.4}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{95.1}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.7}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.4}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.6}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{38.0}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{50.0}\scalebox{0.75}{$\pm$1.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{59.7}\scalebox{0.75}{$\pm$1.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.0}\scalebox{0.75}{$\pm$0.9}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Forget\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{85.2}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{93.0}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{94.5}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{95.1}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{78.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.4}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.0}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{26.4}\scalebox{0.75}{$\pm$1.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{54.3}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.1}\scalebox{0.75}{$\pm$1.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{66.6}\scalebox{0.75}{$\pm$1.1}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}GraNd\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{21.8}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{60.9}\scalebox{0.75}{$\pm$4.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.5}\scalebox{0.75}{$\pm$1.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{18.5}\scalebox{0.75}{$\pm$1.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{25.5}\scalebox{0.75}{$\pm$0.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{49.3}\scalebox{0.75}{$\pm$0.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.0}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{15.5}\scalebox{0.75}{$\pm$1.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{26.0}\scalebox{0.75}{$\pm$1.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{44.7}\scalebox{0.75}{$\pm$1.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{60.4}\scalebox{0.75}{$\pm$1.6}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{\algnamec{}}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{87.9}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.5}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{94.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{95.1}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{83.4}}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.5}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{$\text{\algnamec{}}_B$}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{93.0}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{{19.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{83.6}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.9}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\ \addlinespace[0.1ex]\cline{2-14}\addlinespace[0.1ex]
% \midrule
&\multicolumn{1}{c|}{\hspace{-0.0cm}$\%$ \textit{Improv.}\hspace{-0.10cm}}  
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \algnamec{} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.7\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}5.7\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}6.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.5\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}9.4\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}-6.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}5.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}21.8\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}-6.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}5.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}21.8\%}\end{tabular}
\\
\midrule
% # DivideMix ###############################################################
% # SOP+ ###############################################################
\multirow{8}{*}{\hspace{-0.0cm}{SOP+}\hspace{-0.30cm}}                             
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Uniform\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{87.5}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.5}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.4}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{81.9}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.5}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{{46.5}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.7}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{60.8}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{64.4}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}SmallL\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{77.6}\scalebox{0.75}{$\pm$2.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{86.2}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.7}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{78.8}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{84.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.3}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{48.5}}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{59.8}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{63.9}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{66.1}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Margin\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{52.1}\scalebox{0.75}{$\pm$5.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{79.6}\scalebox{0.75}{$\pm$8.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$3.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.1}\scalebox{0.75}{$\pm$1.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{45.7}\scalebox{0.75}{$\pm$1.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.8}\scalebox{0.75}{$\pm$0.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{84.6}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{92.5}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{20.0}\scalebox{0.75}{$\pm$1.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{34.4}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{50.4}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.3}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}kCenter\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{86.3}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.1}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{95.3}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{81.9}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{88.0}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{91.3}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.3}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{44.8}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.9}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.6}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{65.2}\scalebox{0.75}{$\pm$0.6}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Forget\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{93.0}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{94.2}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.0}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{71.1}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.6}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{38.0}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.2}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{65.8}\scalebox{0.75}{$\pm$0.4}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}GraNd\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{24.2}\scalebox{0.75}{$\pm$5.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{51.6}\scalebox{0.75}{$\pm$3.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{85.9}\scalebox{0.75}{$\pm$1.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.9}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{15.4}\scalebox{0.75}{$\pm$1.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{25.7}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{51.0}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{86.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{11.0}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.0}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{38.7}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{62.1}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{\algnamec{}}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.2}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{93.0}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{94.4}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{83.4}}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{89.3}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{91.5}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{92.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{49.0}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{59.1}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{64.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{65.7}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{$\text{\algnamec{}}_B$}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.6}}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{93.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{94.2}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{95.3}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{84.2}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{89.1}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{91.3}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{92.5}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{52.9}}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{60.1}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{64.1}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{66.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\ \addlinespace[0.1ex]\cline{2-14}\addlinespace[0.1ex]
% \midrule
&\multicolumn{1}{c|}{\hspace{-0.0cm}$\%$ \textit{Improv.}\hspace{-0.10cm}}  
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \algnamec{} }\end{tabular}
%& \begin{tabular}[c]{@{}c@{}}{ - }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}1.3\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}2.8\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}1.5\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}9.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.5\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.3\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
\\
\bottomrule
\end{tabular}
% }
\label{tbl:overall_perf}
% \vspace{-0.5cm}
\end{table*}

